Measuring the Hubble Constant Near and Far in the Era of ELT's

Many of the fundamental physical constants in Physics, as a discipline, are measured to exquisite levels of precision. The fundamental constants that define Cosmology, however, are largely determined via a handful of independent techniques that are applied to even fewer datasets. The history of the measurement of the Hubble Constant (H0), which serves to anchor the expansion history of the Universe to its current value, is an exemplar of the difficulties of cosmological measurement; indeed, as we approach the centennial of its first measurement, the quest for H0 still consumes a great number of resources. In this white paper, we demonstrate how the approaching era of Extremely Large Telescopes (ELTs) will transform the astrophysical measure of H0 from the limited and few into a fundamentally new regime where (i) multiple, independent techniques are employed with modest use of large aperture facilities and (ii) 1% or better precision is readily attainable. This quantum leap in how we approach H0 is due to the unparalleled sensitivity and spatial resolution of ELT's and the ability to use integral field observations for simultaneous spectroscopy and photometry, which together permit both familiar and new techniques to effectively by-pass the conventional 'ladder' framework to minimize total uncertainty. Three independent techniques are discussed -- (i) standard candles via a two-step distance ladder applied to metal, poor stellar populations, (ii) standard clocks via gravitational lens cosmography, and (iii) standard sirens via gravitational wave sources -- each of which can reach 1% with relatively modest investment from 30-m class facilities.

==> h0_elt_decadal.bbl.tex <==

\providecommand{\href}[2]{#2}\begingroup\raggedright\begin{thebibliography}{10}

\bibitem{lemaitre_1927}
G.~{Lema{\^i}tre}, \emph{{Un Univers homog{\`e}ne de masse constante et de
  rayon croissant rendant compte de la vitesse radiale des n{\'e}buleuses
  extra-galactiques}}, {\emph{Annales de la Soci{\'e}t{\'e} Scientifique de
  Bruxelles} {\bfseries 47} (1927) 49}.

\bibitem{hubble_1929}
E.~{Hubble}, \emph{{A Relation between Distance and Radial Velocity among
  Extra-Galactic Nebulae}},
  \href{https://doi.org/10.1073/pnas.15.3.168}{\emph{Proceedings of the
  National Academy of Science} {\bfseries 15} (1929) 168}.

\bibitem{freedman_2001}
W.~L. {Freedman}, B.~F. {Madore}, B.~K. {Gibson}, L.~{Ferrarese}, D.~D.
  {Kelson}, S.~{Sakai} et~al., \emph{{Final Results from the Hubble Space
  Telescope Key Project to Measure the Hubble Constant}},
  \href{https://doi.org/10.1086/320638}{\emph{\apj} {\bfseries 553} (2001) 47}
  [\href{https://arxiv.org/abs/astro-ph/0012376}{{\ttfamily
  astro-ph/0012376}}].

\bibitem{riess_2016}
A.~G. {Riess}, L.~M. {Macri}, S.~L. {Hoffmann}, D.~{Scolnic}, S.~{Casertano},
  A.~V. {Filippenko} et~al., \emph{{A 2.4\% Determination of the Local Value of
  the Hubble Constant}},
  \href{https://doi.org/10.3847/0004-637X/826/1/56}{\emph{\apj} {\bfseries 826}
  (2016) 56} [\href{https://arxiv.org/abs/1604.01424}{{\ttfamily 1604.01424}}].

\bibitem{riess_2018a}
A.~G. {Riess}, S.~{Casertano}, W.~{Yuan}, L.~{Macri}, J.~{Anderson}, J.~W.
  {MacKenty} et~al., \emph{{New Parallaxes of Galactic Cepheids from Spatially
  Scanning the Hubble Space Telescope: Implications for the Hubble Constant}},
  \href{https://doi.org/10.3847/1538-4357/aaadb7}{\emph{\apj} {\bfseries 855}
  (2018) 136} [\href{https://arxiv.org/abs/1801.01120}{{\ttfamily
  1801.01120}}].

\bibitem{riess_2018b}
A.~G. {Riess}, S.~{Casertano}, W.~{Yuan}, L.~{Macri}, B.~{Bucciarelli}, M.~G.
  {Lattanzi} et~al., \emph{{Milky Way Cepheid Standards for Measuring Cosmic
  Distances and Application to Gaia DR2: Implications for the Hubble
  Constant}}, \href{https://doi.org/10.3847/1538-4357/aac82e}{\emph{\apj}
  {\bfseries 861} (2018) 126}
  [\href{https://arxiv.org/abs/1804.10655}{{\ttfamily 1804.10655}}].

\bibitem{bennett_2013}
C.~L. {Bennett}, D.~{Larson}, J.~L. {Weiland}, N.~{Jarosik}, G.~{Hinshaw},
  N.~{Odegard} et~al., \emph{{Nine-year Wilkinson Microwave Anisotropy Probe
  (WMAP) Observations: Final Maps and Results}},
  \href{https://doi.org/10.1088/0067-0049/208/2/20}{\emph{\apjs} {\bfseries
  208} (2013) 20} [\href{https://arxiv.org/abs/1212.5225}{{\ttfamily
  1212.5225}}].

\bibitem{planck_2018}
{Planck Collaboration}, N.~{Aghanim}, Y.~{Akrami}, M.~{Ashdown}, J.~{Aumont},
  C.~{Baccigalupi} et~al., \emph{{Planck 2018 results. VI. Cosmological
  parameters}}, {\emph{arXiv e-prints} (2018) }
  [\href{https://arxiv.org/abs/1807.06209}{{\ttfamily 1807.06209}}].

\bibitem{refsdal_1964}
S.~{Refsdal}, \emph{{On the possibility of determining Hubble's parameter and
  the masses of galaxies from the gravitational lens effect}},
  \href{https://doi.org/10.1093/mnras/128.4.307}{\emph{\mnras} {\bfseries 128}
  (1964) 307}.

\bibitem{schutz_1986}
B.~F. {Schutz}, \emph{{Determining the Hubble constant from gravitational wave
  observations}}, \href{https://doi.org/10.1038/323310a0}{\emph{\nat}
  {\bfseries 323} (1986) 310}.

\bibitem{T+M16}
T.~{Treu} and P.~J. {Marshall}, \emph{{Time delay cosmography}},
  \href{https://doi.org/10.1007/s00159-016-0096-8}{\emph{\aapr} {\bfseries 24}
  (2016) 11} [\href{https://arxiv.org/abs/1605.05333}{{\ttfamily 1605.05333}}].

\bibitem{birrer_2019}
S.~{Birrer}, T.~{Treu}, C.~E. {Rusu}, V.~{Bonvin}, C.~D. {Fassnacht}, J.~H.~H.
  {Chan} et~al., \emph{{H0LiCOW - IX. Cosmographic analysis of the doubly
  imaged quasar SDSS 1206+4332 and a new measurement of the Hubble constant}},
  \href{https://doi.org/10.1093/mnras/stz200}{\emph{\mnras} {\bfseries 484}
  (2019) 4726} [\href{https://arxiv.org/abs/1809.01274}{{\ttfamily
  1809.01274}}].

\bibitem{suyu_2017}
S.~H. {Suyu}, V.~{Bonvin}, F.~{Courbin}, C.~D. {Fassnacht}, C.~E. {Rusu},
  D.~{Sluse} et~al., \emph{{H0LiCOW - I. H$_{0}$ Lenses in COSMOGRAIL's
  Wellspring: program overview}},
  \href{https://doi.org/10.1093/mnras/stx483}{\emph{\mnras} {\bfseries 468}
  (2017) 2590} [\href{https://arxiv.org/abs/1607.00017}{{\ttfamily
  1607.00017}}].

\bibitem{abbott_2017}
B.~P. {Abbott}, R.~{Abbott}, T.~D. {Abbott}, F.~{Acernese}, K.~{Ackley},
  C.~{Adams} et~al., \emph{{A gravitational-wave standard siren measurement of
  the Hubble constant}}, \href{https://doi.org/10.1038/nature24471}{\emph{\nat}
  {\bfseries 551} (2017) 85}
  [\href{https://arxiv.org/abs/1710.05835}{{\ttfamily 1710.05835}}].

\bibitem{freedman_2017}
W.~L. {Freedman}, \emph{{Cosmology at a crossroads}},
  \href{https://doi.org/10.1038/s41550-017-0121}{\emph{Nature Astronomy}
  {\bfseries 1} (2017) 0121}.

\bibitem{aylor_2018}
K.~{Aylor}, M.~{Joy}, L.~{Knox}, M.~{Millea}, S.~{Raghunathan} and W.~L. {Kimmy
  Wu}, \emph{{Sounds Discordant: Classical Distance Ladder \& $\Lambda$CDM
  -based Determinations of the Cosmological Sound Horizon}}, {\emph{arXiv
  e-prints} (2018) } [\href{https://arxiv.org/abs/1811.00537}{{\ttfamily
  1811.00537}}].

\bibitem{poulin_2018}
V.~{Poulin}, T.~L. {Smith}, T.~{Karwal} and M.~{Kamionkowski}, \emph{{Early
  Dark Energy Can Resolve The Hubble Tension}}, {\emph{arXiv e-prints} (2018) }
  [\href{https://arxiv.org/abs/1811.04083}{{\ttfamily 1811.04083}}].

\bibitem{divalentino_2017}
E.~{Di Valentino}, A.~{Melchiorri} and O.~{Mena}, \emph{{Can interacting dark
  energy solve the H$_{0}$ tension?}},
  \href{https://doi.org/10.1103/PhysRevD.96.043503}{\emph{\prd} {\bfseries 96}
  (2017) 043503} [\href{https://arxiv.org/abs/1704.08342}{{\ttfamily
  1704.08342}}].

\bibitem{divalentino_2018}
E.~{Di Valentino}, C.~{B{\oe}hm}, E.~{Hivon} and F.~R. {Bouchet},
  \emph{{Reducing the H$_{0}$ and {$\sigma$}$_{8}$ tensions with dark
  matter-neutrino interactions}},
  \href{https://doi.org/10.1103/PhysRevD.97.043513}{\emph{\prd} {\bfseries 97}
  (2018) 043513} [\href{https://arxiv.org/abs/1710.02559}{{\ttfamily
  1710.02559}}].

\bibitem{kreisch_2019}
C.~D. {Kreisch}, F.-Y. {Cyr-Racine} and O.~{Dor{\'e}}, \emph{{The Neutrino
  Puzzle: Anomalies, Interactions, and Cosmological Tensions}}, {\emph{arXiv
  e-prints} (2019) } [\href{https://arxiv.org/abs/1902.00534}{{\ttfamily
  1902.00534}}].

\bibitem{abazajian_2016}
K.~N. {Abazajian}, P.~{Adshead}, Z.~{Ahmed}, S.~W. {Allen}, D.~{Alonso}, K.~S.
  {Arnold} et~al., \emph{{CMB-S4 Science Book, First Edition}}, {\emph{arXiv
  e-prints} (2016) } [\href{https://arxiv.org/abs/1610.02743}{{\ttfamily
  1610.02743}}].

\bibitem{ade_2019}
P.~{Ade}, J.~{Aguirre}, Z.~{Ahmed}, S.~{Aiola}, A.~{Ali}, D.~{Alonso} et~al.,
  \emph{{The Simons Observatory: science goals and forecasts}},
  \href{https://doi.org/10.1088/1475-7516/2019/02/056}{\emph{\jcap} {\bfseries
  2} (2019) 056} [\href{https://arxiv.org/abs/1808.07445}{{\ttfamily
  1808.07445}}].

\bibitem{beaton_2016}
R.~L. {Beaton}, W.~L. {Freedman}, B.~F. {Madore}, G.~{Bono}, E.~K. {Carlson},
  G.~{Clementini} et~al., \emph{{The Carnegie-Chicago Hubble Program. I. An
  Independent Approach to the Extragalactic Distance Scale Using Only
  Population II Distance Indicators}},
  \href{https://doi.org/10.3847/0004-637X/832/2/210}{\emph{\apj} {\bfseries
  832} (2016) 210} [\href{https://arxiv.org/abs/1604.01788}{{\ttfamily
  1604.01788}}].

\bibitem{riess_2009}
A.~G. {Riess}, L.~{Macri}, S.~{Casertano}, M.~{Sosey}, H.~{Lampeitl}, H.~C.
  {Ferguson} et~al., \emph{{A Redetermination of the Hubble Constant with the
  Hubble Space Telescope from a Differential Distance Ladder}},
  \href{https://doi.org/10.1088/0004-637X/699/1/539}{\emph{\apj} {\bfseries
  699} (2009) 539} [\href{https://arxiv.org/abs/0905.0695}{{\ttfamily
  0905.0695}}].

\bibitem{cassisi_2013}
S.~{Cassisi} and M.~{Salaris}, \emph{{Old Stellar Populations: How to Study the
  Fossil Record of Galaxy Formation}}. Mar., 2013.

\bibitem{serenelli_2017}
A.~{Serenelli}, A.~{Weiss}, S.~{Cassisi}, M.~{Salaris} and A.~{Pietrinferni},
  \emph{{The brightness of the red giant branch tip. Theoretical framework, a
  set of reference models, and predicted observables}},
  \href{https://doi.org/10.1051/0004-6361/201731004}{\emph{\aap} {\bfseries
  606} (2017) A33} [\href{https://arxiv.org/abs/1706.09910}{{\ttfamily
  1706.09910}}].

\bibitem{lee_1993}
M.~G. {Lee}, W.~L. {Freedman} and B.~F. {Madore}, \emph{{The Tip of the Red
  Giant Branch as a Distance Indicator for Resolved Galaxies}},
  \href{https://doi.org/10.1086/173334}{\emph{\apj} {\bfseries 417} (1993)
  553}.

\bibitem{freedman_2010}
W.~L. {Freedman} and B.~F. {Madore}, \emph{{The Hubble Constant}},
  \href{https://doi.org/10.1146/annurev-astro-082708-101829}{\emph{\araa}
  {\bfseries 48} (2010) 673} [\href{https://arxiv.org/abs/1004.1856}{{\ttfamily
  1004.1856}}].

\bibitem{dalcanton_2012}
J.~J. {Dalcanton}, B.~F. {Williams}, J.~L. {Melbourne}, L.~{Girardi},
  A.~{Dolphin}, P.~A. {Rosenfield} et~al., \emph{{Resolved Near-infrared
  Stellar Populations in Nearby Galaxies}},
  \href{https://doi.org/10.1088/0067-0049/198/1/6}{\emph{\apjs} {\bfseries 198}
  (2012) 6} [\href{https://arxiv.org/abs/1109.6893}{{\ttfamily 1109.6893}}].

\bibitem{beaton_2018}
R.~L. {Beaton}, G.~{Bono}, V.~F. {Braga}, M.~{Dall'Ora}, G.~{Fiorentino}, I.~S.
  {Jang} et~al., \emph{{Old-Aged Primary Distance Indicators}},
  \href{https://doi.org/10.1007/s11214-018-0542-1}{\emph{\ssr} {\bfseries 214}
  (2018) 113}.

\bibitem{jang_2018}
I.~S. {Jang}, D.~{Hatt}, R.~L. {Beaton}, M.~G. {Lee}, W.~L. {Freedman}, B.~F.
  {Madore} et~al., \emph{{The Carnegie-Chicago Hubble Program. III. The
  Distance to NGC 1365 via the Tip of the Red Giant Branch}},
  \href{https://doi.org/10.3847/1538-4357/aa9d92}{\emph{\apj} {\bfseries 852}
  (2018) 60} [\href{https://arxiv.org/abs/1703.10616}{{\ttfamily 1703.10616}}].

\bibitem{hatt_2018a}
D.~{Hatt}, W.~L. {Freedman}, B.~F. {Madore}, R.~L. {Beaton}, T.~J. {Hoyt},
  I.~S. {Jang} et~al., \emph{{The Carnegie-Chicago Hubble Program. IV. The
  Distance to NGC 4424, NGC 4526, and NGC 4356 via the Tip of the Red Giant
  Branch}}, \href{https://doi.org/10.3847/1538-4357/aac9cc}{\emph{\apj}
  {\bfseries 861} (2018) 104}
  [\href{https://arxiv.org/abs/1806.02900}{{\ttfamily 1806.02900}}].

\bibitem{hatt_2018b}
D.~{Hatt}, W.~L. {Freedman}, B.~F. {Madore}, I.~S. {Jang}, R.~L. {Beaton},
  T.~J. {Hoyt} et~al., \emph{{The Carnegie Chicago Hubble Program. V. The
  Distances to NGC 1448 and NGC 1316 via the Tip of the Red Giant Branch}},
  \href{https://doi.org/10.3847/1538-4357/aadfe8}{\emph{\apj} {\bfseries 866}
  (2018) 145} [\href{https://arxiv.org/abs/1809.01741}{{\ttfamily
  1809.01741}}].

\bibitem{hatt_2017}
D.~{Hatt}, R.~L. {Beaton}, W.~L. {Freedman}, B.~F. {Madore}, I.-S. {Jang},
  T.~J. {Hoyt} et~al., \emph{{The Carnegie-Chicago Hubble Program. II. The
  Distance to IC 1613: The Tip of the Red Giant Branch and RR Lyrae
  Period-luminosity Relations}},
  \href{https://doi.org/10.3847/1538-4357/aa7f73}{\emph{\apj} {\bfseries 845}
  (2017) 146} [\href{https://arxiv.org/abs/1703.06468}{{\ttfamily
  1703.06468}}].

\bibitem{madore_2018}
B.~F. {Madore}, W.~L. {Freedman}, D.~{Hatt}, T.~J. {Hoyt}, A.~J. {Monson},
  R.~L. {Beaton} et~al., \emph{{The Near-infrared Tip of the Red Giant Branch.
  I. A Calibration in the Isolated Dwarf Galaxy IC 1613}},
  \href{https://doi.org/10.3847/1538-4357/aab7f4}{\emph{\apj} {\bfseries 858}
  (2018) 11} [\href{https://arxiv.org/abs/1803.01278}{{\ttfamily 1803.01278}}].

\bibitem{hoyt_2018}
T.~J. {Hoyt}, W.~L. {Freedman}, B.~F. {Madore}, M.~{Seibert}, R.~L. {Beaton},
  D.~{Hatt} et~al., \emph{{The Near-infrared Tip of the Red Giant Branch. II.
  An Absolute Calibration in the Large Magellanic Cloud}},
  \href{https://doi.org/10.3847/1538-4357/aab7ed}{\emph{\apj} {\bfseries 858}
  (2018) 12} [\href{https://arxiv.org/abs/1803.01277}{{\ttfamily 1803.01277}}].

\bibitem{tully_2016}
R.~B. {Tully}, H.~M. {Courtois} and J.~G. {Sorce}, \emph{{Cosmicflows-3}},
  \href{https://doi.org/10.3847/0004-6256/152/2/50}{\emph{\aj} {\bfseries 152}
  (2016) 50} [\href{https://arxiv.org/abs/1605.01765}{{\ttfamily 1605.01765}}].

\bibitem{lee_2014}
C.-H. {Lee}, J.~{Koppenhoefer}, S.~{Seitz}, R.~{Bender}, A.~{Riffeser},
  M.~{Kodric} et~al., \emph{{Properties of M31. V. 298 Eclipsing Binaries from
  PAndromeda}}, \href{https://doi.org/10.1088/0004-637X/797/1/22}{\emph{\apj}
  {\bfseries 797} (2014) 22} [\href{https://arxiv.org/abs/1411.1115}{{\ttfamily
  1411.1115}}].

\bibitem{vilardell_2010}
F.~{Vilardell}, I.~{Ribas}, C.~{Jordi}, E.~L. {Fitzpatrick} and E.~F. {Guinan},
  \emph{{The distance to the Andromeda galaxy from eclipsing binaries}},
  \href{https://doi.org/10.1051/0004-6361/200913299}{\emph{\aap} {\bfseries
  509} (2010) A70} [\href{https://arxiv.org/abs/0911.3391}{{\ttfamily
  0911.3391}}].

\bibitem{pietrzynski_2013}
G.~{Pietrzy{\'n}ski}, D.~{Graczyk}, W.~{Gieren}, I.~B. {Thompson},
  B.~{Pilecki}, A.~{Udalski} et~al., \emph{{An eclipsing-binary distance to the
  Large Magellanic Cloud accurate to two per cent}},
  \href{https://doi.org/10.1038/nature11878}{\emph{\nat} {\bfseries 495} (2013)
  76} [\href{https://arxiv.org/abs/1303.2063}{{\ttfamily 1303.2063}}].

\bibitem{graczyk_2018}
D.~{Graczyk}, G.~{Pietrzy{\'n}ski}, I.~B. {Thompson}, W.~{Gieren},
  B.~{Pilecki}, P.~{Konorski} et~al., \emph{{The Late-type Eclipsing Binaries
  in the Large Magellanic Cloud: Catalog of Fundamental Physical Parameters}},
  \href{https://doi.org/10.3847/1538-4357/aac2bf}{\emph{\apj} {\bfseries 860}
  (2018) 1} [\href{https://arxiv.org/abs/1805.04952}{{\ttfamily 1805.04952}}].

\bibitem{courbin_2018}
F.~{Courbin}, V.~{Bonvin}, E.~{Buckley-Geer}, C.~D. {Fassnacht}, J.~{Frieman},
  H.~{Lin} et~al., \emph{{COSMOGRAIL: the COSmological MOnitoring of
  GRAvItational Lenses. XVI. Time delays for the quadruply imaged quasar DES
  J0408-5354 with high-cadence photometric monitoring}},
  \href{https://doi.org/10.1051/0004-6361/201731461}{\emph{\aap} {\bfseries
  609} (2018) A71}.

\bibitem{falco_1985}
E.~E. {Falco}, M.~V. {Gorenstein} and I.~I. {Shapiro}, \emph{{On
  model-dependent bounds on H(0) from gravitational images Application of Q0957
  + 561A,B}}, \href{https://doi.org/10.1086/184422}{\emph{\apjl} {\bfseries
  289} (1985) L1}.

\bibitem{shajib_2018}
A.~J. {Shajib}, T.~{Treu} and A.~{Agnello}, \emph{{Improving time-delay
  cosmography with spatially resolved kinematics}},
  \href{https://doi.org/10.1093/mnras/stx2302}{\emph{\mnras} {\bfseries 473}
  (2018) 210} [\href{https://arxiv.org/abs/1709.01517}{{\ttfamily
  1709.01517}}].

\bibitem{goobar_2017}
A.~{Goobar}, R.~{Amanullah}, S.~R. {Kulkarni}, P.~E. {Nugent}, J.~{Johansson},
  C.~{Steidel} et~al., \emph{{iPTF16geu: A multiply imaged, gravitationally
  lensed type Ia supernova}},
  \href{https://doi.org/10.1126/science.aal2729}{\emph{Science} {\bfseries 356}
  (2017) 291} [\href{https://arxiv.org/abs/1611.00014}{{\ttfamily
  1611.00014}}].

\bibitem{aihara_2018}
H.~{Aihara}, N.~{Arimoto}, R.~{Armstrong}, S.~{Arnouts}, N.~A. {Bahcall},
  S.~{Bickerton} et~al., \emph{{The Hyper Suprime-Cam SSP Survey: Overview and
  survey design}}, \href{https://doi.org/10.1093/pasj/psx066}{\emph{\pasj}
  {\bfseries 70} (2018) S4} [\href{https://arxiv.org/abs/1704.05858}{{\ttfamily
  1704.05858}}].

\bibitem{Oguri_2010}
M.~{Oguri} and P.~J. {Marshall}, \emph{{Gravitationally lensed quasars and
  supernovae in future wide-field optical imaging surveys}},
  \href{https://doi.org/10.1111/j.1365-2966.2010.16639.x}{\emph{\mnras}
  {\bfseries 405} (2010) 2579}
  [\href{https://arxiv.org/abs/1001.2037}{{\ttfamily 1001.2037}}].

\bibitem{goldstein_2017}
D.~A. {Goldstein} and P.~E. {Nugent}, \emph{{How to Find Gravitationally Lensed
  Type Ia Supernovae}},
  \href{https://doi.org/10.3847/2041-8213/834/1/L5}{\emph{\apjl} {\bfseries
  834} (2017) L5} [\href{https://arxiv.org/abs/1611.09459}{{\ttfamily
  1611.09459}}].

\bibitem{holz_2005}
D.~E. {Holz} and S.~A. {Hughes}, \emph{{Using Gravitational-Wave Standard
  Sirens}}, \href{https://doi.org/10.1086/431341}{\emph{\apj} {\bfseries 629}
  (2005) 15} [\href{https://arxiv.org/abs/astro-ph/0504616}{{\ttfamily
  astro-ph/0504616}}].

\bibitem{chen_2018}
H.-Y. {Chen}, M.~{Fishbach} and D.~E. {Holz}, \emph{{A two per cent Hubble
  constant measurement from standard sirens within five years}},
  \href{https://doi.org/10.1038/s41586-018-0606-0}{\emph{\nat} {\bfseries 562}
  (2018) 545} [\href{https://arxiv.org/abs/1712.06531}{{\ttfamily
  1712.06531}}].

\bibitem{massari_2016}
D.~{Massari}, G.~{Fiorentino}, A.~{McConnachie}, A.~{Bellini}, E.~{Tolstoy},
  P.~{Turri} et~al., \emph{{Astrometry with MCAO: HST-GeMS proper motions in
  the globular cluster NGC 6681}},
  \href{https://doi.org/10.1051/0004-6361/201629336}{\emph{\aap} {\bfseries
  595} (2016) L2} [\href{https://arxiv.org/abs/1609.05923}{{\ttfamily
  1609.05923}}].

\bibitem{turri_2016}
P.~{Turri}, A.~W. {McConnachie}, P.~B. {Stetson}, D.~R. {Andersen}, J.-P.
  {V{\'e}ran}, G.~{Fiorentino} et~al., \emph{{Photometric techniques,
  performance and PSF characterization of GeMS}},  in \emph{Adaptive Optics
  Systems V}, vol.~9909 of \emph{\procspie}, p.~990907, July, 2016,
  \href{https://doi.org/10.1117/12.2233109}{DOI}.

\bibitem{saha_2014}
A.~{Saha}, T.~{Matheson}, R.~{Snodgrass}, J.~{Kececioglu}, G.~{Narayan},
  R.~{Seaman} et~al., \emph{{ANTARES: a prototype transient broker system}},
  in \emph{Observatory Operations: Strategies, Processes, and Systems V},
  vol.~9149 of \emph{\procspie}, p.~914908, July, 2014,
  \href{https://arxiv.org/abs/1409.0056}{{\ttfamily 1409.0056}},
  \href{https://doi.org/10.1117/12.2056988}{DOI}.

\end{thebibliography}\endgroup

